Certified homotopy tracking using the Krawczyk method

We revisit the problem of certifying the correctness of approximate solution paths computed by numerical homotopy continuation methods. We propose a conceptually simple approach based on a parametric variant of the Krawczyk method from interval arithmetic. Unlike most previous methods for certified path-tracking, our approach is applicable in the general setting of parameter homotopies commonly used to solve polynomial systems of equations. We also describe a novel preconditioning strategy and give theoretical correctness and termination results. Experiments using a preliminary implementation of the method indicate that our approach is competitive with specialized methods appearing previously in the literature, in spite of our more general setting.

==> figure1.tex <==

\begin{tikzpicture}[rotate around x=0,rotate around y=45, rotate around z=0,scale=.8]
%the first box
\draw[line width=0.5mm,thick,color=red] (1,1.5,4.5) -- (2,2,4.5);
\draw[line width=0.5mm,thick,color=red] (4,1,4.5) -- (2,2,4.5);

\draw[line width=0.2mm] (1,1,5) -- (2,1.5,5);
\draw[line width=0.2mm] (1,1,5) -- (1,2,5);
\draw[line width=0.2mm] (2,2.5,5) -- (1,2,5);
\draw[line width=0.2mm] (2,2.5,5) -- (2,1.5,5);
\draw (1,1.5,4.5) node {$\bullet$};

\draw[line width=0.2mm] (1,2,5) -- (1,2,4);
\draw[line width=0.2mm] (2,2.5,4) -- (1,2,4);
\draw[line width=0.2mm] (2,2.5,4) -- (2,2.5,5);
\draw[line width=0.2mm] (1,1,4) -- (1,1,5);
\draw (2,2,4.5) node {$\bullet$};


\draw[line width=0.2mm] (1,1,4) -- (1,2,4);
\draw[line width=0.2mm] (1,1,4) -- (1,1,5);
\draw[line width=0.3mm,dashed] (2,1.5,5) -- (2,1.5,4);
\draw[line width=0.3mm,dashed] (2,2.5,4) -- (2,1.5,4);
\draw[line width=0.3mm,dashed] (2,1.5,4) -- (1,1,4);


%the second box
\draw[line width=0.2mm] (2,3,3.5) -- (2,3,5.5);
\draw[line width=0.2mm] (2,1,5.5) -- (2,3,5.5);
\draw[line width=0.3mm,dotted] (2,1,4.2) -- (2,1,3.5);
\draw[line width=0.2mm] (2,1,4.2) -- (2,1,5.5);
\draw[line width=0.2mm] (2,3,3.5) -- (2,2.2,3.5);
\draw[line width=0.3mm,dotted] (2,2.2,3.5) -- (2,1,3.5);

\draw[line width=0.2mm] (2,1,5.5) -- (4,0,5.5);
\draw[line width=0.2mm] (2,3,5.5) -- (4,2,5.5);
\draw[line width=0.2mm] (4,0,5.5) -- (4,2,5.5);

\draw[line width=0.2mm] (2,3,3.5) -- (4,2,3.5);
\draw[line width=0.2mm] (4,2,5.5) -- (4,2,3.5);
\draw[line width=0.3mm,dotted] (4,2,3.5) -- (4,0,3.5);
\draw[line width=0.3mm,dotted] (4,0,5.5) -- (4,0,3.5);
\draw[line width=0.3mm,dotted] (2,1,3.5) -- (4,0,3.5);
\draw (4,1,4.5) node {$\bullet$};




%\draw (6,2,4.5) node {$\bullet$};

\draw[line width=.4mm]
plot[variable=\x,domain=.5:5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);
\draw[line width=.4mm,dotted]
plot[variable=\x,domain=.4:.5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);
\draw[line width=.4mm,dotted]
plot[variable=\x,domain=5:5.5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);

\draw[line width=0.4mm,dotted] (2,1.5,5) -- (2,0,5);
\draw[line width=0.4mm,dotted] (1,1,5) -- (1,0,5);

\draw[line width=0.3mm,dashed] (1,0,7) -- (1,0,5);
\draw[line width=0.3mm,dashed] (2,0,7) -- (2,0,5);
\draw[line width=0.3mm,dashed] (4,0,7) -- (4,0,5.5);


\draw[->,line width=0.1mm] (-1.5,0,7) -- (6.5,0,7);
\draw (6.5,-.1,7.3) node {$t$};


\draw (-1,0,7) node {$\bullet$};
\draw (-1,-.15,7.3) node {$t=1$};

\draw (.9,-.1,7.5) node {$t_{i-1}$};
\draw (2.3,-.1,8) node {$t_i=t_{i-1}-dt$};
\draw (4.3,-.1,8) node {$t_{i+1}=t_{i}-\lambda dt$};
\draw (5.7,0,7) node {$\bullet$};
\draw (5.7,-.15,7.3) node {$t=0$};









\end{tikzpicture}


==> figure2.tex <==

\begin{tikzpicture}[rotate around x=0,rotate around y=45, rotate around z=0,scale=.8]
%the first box
\draw[line width=0.5mm,thick,color=red] (1,1.5,4.5) -- (2,2,4.5);
\draw[line width=0.5mm,thick,color=red] (4,1,4.5) -- (2,2,4.5);

\draw[line width=0.2mm] (1,1,5) -- (2,1.5,5);
\draw[line width=0.2mm] (1,1,5) -- (1,2,5);
\draw[line width=0.2mm] (2,2.5,5) -- (1,2,5);
\draw[line width=0.2mm] (2,2.5,5) -- (2,1.5,5);
\draw (1,1.5,4.5) node {$\bullet$};

\draw[line width=0.2mm] (1,2,5) -- (1,2,4);
\draw[line width=0.2mm] (2,2.5,4) -- (1,2,4);
\draw[line width=0.2mm] (2,2.5,4) -- (2,2.5,5);
\draw[line width=0.2mm] (1,1,4) -- (1,1,5);
\draw (2,2,4.5) node {$\bullet$};


\draw[line width=0.2mm] (1,1,4) -- (1,2,4);
\draw[line width=0.2mm] (1,1,4) -- (1,1,5);
\draw[line width=0.3mm,dashed] (2,1.5,5) -- (2,1.5,4);
\draw[line width=0.3mm,dashed] (2,2.5,4) -- (2,1.5,4);
\draw[line width=0.3mm,dashed] (2,1.5,4) -- (1,1,4);


%the second box
\draw[line width=0.2mm] (2,3,3.5) -- (2,3,5.5);
\draw[line width=0.2mm] (2,1,5.5) -- (2,3,5.5);
\draw[line width=0.3mm,dotted] (2,1,4.2) -- (2,1,3.5);
\draw[line width=0.2mm] (2,1,4.2) -- (2,1,5.5);
\draw[line width=0.2mm] (2,3,3.5) -- (2,2.2,3.5);
\draw[line width=0.3mm,dotted] (2,2.2,3.5) -- (2,1,3.5);

\draw[line width=0.2mm] (2,1,5.5) -- (4,0,5.5);
\draw[line width=0.2mm] (2,3,5.5) -- (4,2,5.5);
\draw[line width=0.2mm] (4,0,5.5) -- (4,2,5.5);

\draw[line width=0.2mm] (2,3,3.5) -- (4,2,3.5);
\draw[line width=0.2mm] (4,2,5.5) -- (4,2,3.5);
\draw[line width=0.3mm,dotted] (4,2,3.5) -- (4,0,3.5);
\draw[line width=0.3mm,dotted] (4,0,5.5) -- (4,0,3.5);
\draw[line width=0.3mm,dotted] (2,1,3.5) -- (4,0,3.5);
\draw (4,1,4.5) node {$\bullet$};




%\draw (6,2,4.5) node {$\bullet$};

\draw[line width=.4mm]
plot[variable=\x,domain=.5:5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);
\draw[line width=.4mm,dotted]
plot[variable=\x,domain=.4:.5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);
\draw[line width=.4mm,dotted]
plot[variable=\x,domain=5:5.5,samples=73,smooth] 
 (\x,{7/60 *\x^3-23/20 *\x^2+47/15*\x-3/5},4.5);

\draw[line width=0.4mm,dotted] (2,1.5,5) -- (2,0,5);
\draw[line width=0.4mm,dotted] (1,1,5) -- (1,0,5);

\draw[line width=0.3mm,dashed] (1,0,7) -- (1,0,5);
\draw[line width=0.3mm,dashed] (2,0,7) -- (2,0,5);
\draw[line width=0.3mm,dashed] (4,0,7) -- (4,0,5.5);


\draw[->,line width=0.1mm] (-1.5,0,7) -- (6.5,0,7);
\draw (6.5,-.1,7.3) node {$t$};


\draw (-1,0,7) node {$\bullet$};
\draw (-1,-.15,7.3) node {$t=1$};

\draw (.9,-.1,7.5) node {$t_{i-1}$};
\draw (2.3,-.1,8) node {$t_i=t_{i-1}-dt$};
\draw (4.3,-.1,8) node {$t_{i+1}=t_{i}-\lambda dt$};
\draw (5.7,0,7) node {$\bullet$};
\draw (5.7,-.15,7.3) node {$t=0$};









\end{tikzpicture}

